A Game-Theoretic Approach for Adversarial Information Fusion in Distributed Sensor Networks

Every day we share our personal information through digital systems which are constantly exposed to threats. For this reason, security-oriented disciplines of signal processing have received increasing attention in the last decades: multimedia forensics, digital watermarking, biometrics, network monitoring, steganography and steganalysis are just a few examples. Even though each of these fields has its own peculiarities, they all have to deal with a common problem: the presence of one or more adversaries aiming at making the system fail. Adversarial Signal Processing lays the basis of a general theory that takes into account the impact that the presence of an adversary has on the design of effective signal processing tools. By focusing on the application side of Adversarial Signal Processing, namely adversarial information fusion in distributed sensor networks, and adopting a game-theoretic approach, this thesis contributes to the above mission by addressing four issues. First, we address decision fusion in distributed sensor networks by developing a novel soft isolation defense scheme that protect the network from adversaries, specifically, Byzantines. Second, we develop an optimum decision fusion strategy in the presence of Byzantines. In the next step, we propose a technique to reduce the complexity of the optimum fusion by relying on a novel near-optimum message passing algorithm based on factor graphs. Finally, we introduce a defense mechanism to protect decentralized networks running consensus algorithm against data falsification attacks.

==> acknowledgements.tex <==

%%% Chapter heading commands %%%

\chapter*{Acknowledgements}
\markboth{Acknowledgements}{}

\bigskip

\PARstart{\color{red}I} would like to express my gratitude to my advisor Professor Mauro Barni for his guidance during my Ph.D studies, for his motivation, enthusiasm and knowledge. I also thank him for the support to my work and for his efforts to make me a good researcher. Also I would like to thank my
co-supervisor Professor Andrea Abrardo for his effort and guidance. Additionally, I wish to thank the thesis reviewers and members of the committee, Professor Vincenzo Matta (University of Salerno) and Professor Vito 
Fragnelli (University of Piemonte Orientale), for their
insightful comments and suggestions.

I would like to thank all of my laboratory colleagues in Siena for their support and help: Benedetta, Riccardo, Andrea, Giulia and Tommaso. A special thanks go to
Benedetta Tondi and Riccardo Lazzeretti who shared with me the intuition and the research work
that led to many scientific publications. Working with them has been a great and exciting experience.

Since I deeply believe that what a man does in his job is just an expression of who he is, I want to thank all those persons who contribute to my education:
My mother and father for all their effort and patience to make us what we are now, my sister Batoul, my sister and little angel Maya and my brother Engineer Ali Kallas who always encouraged me and support me during my studies, I thank him for all his efforts. Last but not the least, I want to thank my friends, especially those in Siena, Nasim Omidian Sijani, the wonderful person who supported and encouraged me, I thank her for all the time we spent together, and Alaa Krayim for his friendship, he is one of the best people I have ever known in this city, Siena.

\begin{flushright}
Siena
\\
01/03/2017
\end{flushright}

